Calibrating Multimodal Learning

Multimodal machine learning has achieved remarkable progress in a wide range of scenarios. However, the reliability of multimodal learning remains largely unexplored. In this paper, through extensive empirical studies, we identify current multimodal classification methods suffer from unreliable predictive confidence that tend to rely on partial modalities when estimating confidence. Specifically, we find that the confidence estimated by current models could even increase when some modalities are corrupted. To address the issue, we introduce an intuitive principle for multimodal learning, i.e., the confidence should not increase when one modality is removed. Accordingly, we propose a novel regularization technique, i.e., Calibrating Multimodal Learning (CML) regularization, to calibrate the predictive confidence of previous methods. This technique could be flexibly equipped by existing models and improve the performance in terms of confidence calibration, classification accuracy, and model robustness.

==> tabs/appdix-tabs/animaltype1.tex <==
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type I).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{CMA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.1}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.2}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.3}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.4}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}
\\ \midrule 
\multirow{7}{*} {\textbf{Animal}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark                                                                &80.78$\pm$2.79   &80.96$\pm$2.78   &80.85$\pm$2.80        &80.81$\pm$2.88       &80.68$\pm$2.93                           \\
                                                                                 &             & \cmark                                                                                                       &\textbf{82.03$\pm$1.91}  &\textbf{82.37$\pm$2.09}   &\textbf{82.55$\pm$2.24}   &\textbf{82.42$\pm$2.22}        &\textbf{82.30$\pm$2.40}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark                                                              &80.70$\pm$2.45  &79.81$\pm$3.14   &77.34$\pm$4.80   &72.89$\pm$7.46        &68.52$\pm$9.68    \\
                                                            &                       & \cmark                             &\textbf{82.07$\pm$1.57}  &\textbf{81.23$\pm$2.32}   &\textbf{78.93$\pm$3.65}   &\textbf{75.81$\pm$6.30}        &\textbf{72.39$\pm$8.35}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark                                                                &80.87$\pm$2.55   &79.97$\pm$3.12   &77.11$\pm$5.86        &72.23$\pm$9.04 &65.08$\pm$12.75                                 \\
                                                                                 &             & \cmark                                                                 &\textbf{82.14$\pm$1.76}
                                          &\textbf{81.95$\pm$2.65}               &\textbf{79.63$\pm$5.28}   &\textbf{76.63$\pm$7.73}   &\textbf{72.46$\pm$11.39}                 \\   \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tabs/appdix-tabs/animaltype2.tex <==
%Animal
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type II).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{CMA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.5}$\\ \end{tabular}}
\\ \midrule
\multirow{7}{*} {\textbf{Animal}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark          &86.61$\pm$0.20  &85.81$\pm$0.36   &84.82$\pm$1.02   &83.77$\pm$1.29        &82.16$\pm$2.32                                  \\
                                                                                 &             & \cmark                &\textbf{87.20$\pm$0.18}   &\textbf{87.01$\pm$0.18}   &\textbf{86.60$\pm$0.20}        &\textbf{86.03$\pm$0.04}  &\textbf{85.42$\pm$0.29}                                      \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark          &86.33$\pm$0.54  &85.62$\pm$0.61   &84.84$\pm$0.95   &83.04$\pm$1.24        &81.34$\pm$1.73    \\
                                                                                  
                                                            &                           & \cmark                                                                                   &\textbf{87.04$\pm$0.08}   &\textbf{86.64$\pm$0.26}   &\textbf{85.95$\pm$0.42}        &\textbf{84.78$\pm$0.17}  &\textbf{82.71$\pm$0.24}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &86.01$\pm$0.17  &84.80$\pm$0.81  &83.17$\pm$1.65  &80.92$\pm$2.77   &77.42$\pm$4.14                                         \\
                                                                                 &             & \cmark                                                     &\textbf{87.04$\pm$0.42}  &\textbf{86.50$\pm$0.15}   &\textbf{85.38$\pm$0.34}   &\textbf{83.84$\pm$0.65}       &\textbf{81.67$\pm$0.75}                                                                                                      \\ 
                                                    \bottomrule
\end{tabular}

\end{center}
\end{table}

==> tabs/appdix-tabs/bayesian.tex <==
\begin{table}[ht]
\vskip 0.15in
\begin{center}
% \begin{spacing}{1.35}   
% \footnotesize
\caption{Accuracy performance comparison for whether the model is equipped with the CML regularization term (i.e., whether $\lambda$ is set to 0).}
\label{tab:bayesian}
\center
\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{1.75mm}
\begin{tabular}{c|c|ccccc}
\toprule
\multicolumn{1}{c}{\text{Method}}  & \multicolumn{1}{c}{\text{Dataset}}  & \text{CML}  & \text{\begin{tabular}[c]{@{}c@{}}Accuracy\\ ($\uparrow$)\end{tabular}} & \text{\begin{tabular}[c]{@{}c@{}}NLL\\ ($\downarrow$)\end{tabular}} & \text{\begin{tabular}[c]{@{}c@{}}AURC\\ ($\downarrow$)\end{tabular}}& \text{\begin{tabular}[c]{@{}c@{}}E-AURC\\ ($\downarrow$)\end{tabular}} \\ \midrule 
\multirow{10}{*} {\text{Type I}}         
     &  \multirow{3}{*}{\text{CUB}}      & \xmark          &$87.00\pm4.36$                                                    &$20.49\pm0.30$  &$59.44\pm22.10$   &$49.52\pm17.35$                         \\
                                                                                 &             & \cmark                                                    &${88.33\pm4.05}$                                                    &${20.53\pm0.46}$  &${55.94\pm17.07}$   &${47.92\pm16.89}$       \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 1.33 $}} & \textcolor{mycolor1}{{$~~~~~~~~\bigtriangledown 0.04 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.50 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 1.60 $}}                                          \\ \cmidrule{2-7}
    
     &  \multirow{3}{*}{\text{Animal}}      & \xmark          &$81.72\pm2.51$                                                    &$36.87\pm0.41$  &$82.14\pm27.20$   &$63.94\pm22.74$                              \\
                                                                                 &             & \cmark                                                    &${82.73\pm1.64}$                                                    &$36.87\pm0.36$  &${71.54\pm16.03}$   &${55.50\pm13.13}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 1.01 $}} & ${-}$& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 10.60 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 8.44 $}}     \\ \cmidrule{2-7}
     &  \multirow{3}{*}{\shortstack{\text{TUAND-}\\\text{ROMD}}}      & \xmark          &$84.66\pm0.43$                                                    &$6.88\pm0.00$  &$61.46\pm6.09$   &$49.00\pm5.75$                                            \\
                                                                                 &             & \cmark                                                    &${85.20\pm0.81}$                                                   &${6.88\pm0.00}$  &${58.24\pm5.05}$   &${46.64\pm4.55}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.54 $}} & ${-}$& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.22 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 2.36 $}}                                                       \\ \midrule
\multirow{10}{*} {\text{Type II}}    
     
     &  \multirow{3}{*}{\text{CUB}}      & \xmark          &$92.33\pm1.11$                                                    &$2.33\pm0.55$  &$10.92\pm1.94$   &$7.82\pm1.32$                    \\
                                                                                 &             & \cmark                                                    &${94.50\pm1.71}$                                                    &${2.24\pm1.27}$  &${9.32\pm3.91}$   &${7.60\pm3.02}$        \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 2.17 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 0.86 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 1.60 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 0.22 $}}                                        \\ \cmidrule{2-7}
    
     &  \multirow{3}{*}{\text{Animal}}      & \xmark          &$86.75\pm0.33$                                                  &$8.25\pm3.79$  &$27.62\pm7.42$   &$18.40\pm7.27$               \\
                                                                                 &             & \cmark                                                    &${87.61\pm0.50}$                                                    &${4.99\pm0.46}$  &${21.26\pm1.31}$   &${13.24\pm0.92}$     \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.86 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.26 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.36 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 5.16 $}} \\ \cmidrule{2-7}
     &  \multirow{3}{*}{\shortstack{\text{TUAND-}\\\text{ROMD}}}      & \xmark          &$86.32\pm0.85$                                                    &$3.26\pm0.09$  &$43.40\pm2.65$   &$33.56\pm2.38$               \\
                                                                                 &             & \cmark                                                    &${88.69\pm0.99}$                                                    &${3.21\pm0.15}$  &${38.62\pm5.44}$   &${31.90\pm4.37}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 2.37 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 0.05 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 4.78 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 1.66 $}}                                                        \\
       \midrule
\multirow{7}{*} {\text{Type III}}    
     
     &  \multirow{3}{*}{\text{NYUD2}}      & \xmark          &$66.89\pm0.85$                                                    &$10.03\pm0.10$  &$140.53\pm5.66$   &$78.40\pm5.01$                    \\
                                                                                 &             & \cmark                                                    &${68.09\pm0.68}$                                                    &${9.83\pm0.15}$  &${137.27\pm6.94}$   &${79.87\pm6.30}$        \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 1.20 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 0.20 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 3.26 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 1.47 $}}
                                                                                 
                                                                                 \\
                                                                                 
                                                                        \cmidrule{2-7}
     &  \multirow{3}{*}{\shortstack{\text{SUN-}\\\text{RGBD}}}      & \xmark          &$62.11\pm0.31$                                                    &$13.27\pm0.53$  &$181.00\pm1.20$   &$97.87\pm1.48$               \\
                                                                                 &             & \cmark                                                    &${62.78\pm0.32}$                                                    &${13.25\pm0.46}$  &${174.90\pm1.50}$   &${95.00\pm1.00}$   \\& & Improve & \textcolor{mycolor2}{{$~~~~~~~~\bigtriangleup 0.67 $}} & \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 0.05 $}}& \textcolor{mycolor2}{{$~~~~~~\bigtriangleup 6.10 $}}& \textcolor{mycolor2}{{$~~~~~~~\bigtriangleup 2.87 $}}                                                        \\
                                                                                 \bottomrule
\end{tabular}}
% \end{spacing}
\end{center}
\end{table}





==> tabs/appdix-tabs/cubtype1.tex <==
%CUB
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type I).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{CMA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.1}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.2}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.3}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.4}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}
\\ \midrule 
\multirow{7}{*} {\textbf{CUB}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark                                                              &84.72$\pm$3.32  &82.22$\pm$4.53   &79.72$\pm$4.43   &76.39$\pm$6.85        &71.17$\pm$9.14                                  \\
                                                                                 &             & \cmark                              &\textbf{85.83$\pm$2.72}   &\textbf{85.00$\pm$3.50}   &\textbf{84.17$\pm$4.08}        &\textbf{83.06$\pm$3.99}  &\textbf{81.11$\pm$4.37}                                      \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark                                                              &84.44$\pm$2.75  &83.89$\pm$3.22   &83.61$\pm$2.83   &83.89$\pm$3.49        &83.61$\pm$3.87    \\
                                                                                  
                                                            &                           & \cmark                                                                                                  &\textbf{85.83$\pm$3.40}   &\textbf{85.28$\pm$2.75}   &\textbf{85.28$\pm$1.97}        &\textbf{85.28$\pm$1.97}  &\textbf{85.00$\pm$1.80}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark                                                              &85.00$\pm$3.12  &82.78$\pm$3.98  &80.00$\pm$4.46  &76.67$\pm$7.48   &72.50$\pm$11.14                                         \\
                                                                                 &             & \cmark                                                                                                        &\textbf{85.83$\pm$2.72}  &\textbf{85.84$\pm$3.12}   &\textbf{85.83$\pm$4.25}   &\textbf{84.44$\pm$4.38}       &\textbf{81.39$\pm$6.43}                                                                                                      \\ 
                                                    \bottomrule
\end{tabular}

\end{center}
\end{table}

==> tabs/appdix-tabs/cubtype2.tex <==
%CUB-type2
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type II).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{CMA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.5}$\\ \end{tabular}}
\\ \midrule
\multirow{7}{*} {\textbf{CUB}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark &91.11$\pm$1.04  &86.94$\pm$2.83   &83.61$\pm$3.93   &80.83$\pm$4.14        &79.17$\pm$3.79                                  \\
                                                                                 &             & \cmark   &\textbf{93.33$\pm$1.80}   &\textbf{90.83$\pm$2.45}   &\textbf{87.50$\pm$3.60}        &\textbf{85.56$\pm$4.38}  &\textbf{81.11$\pm$4.53}                                      \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark          &91.11$\pm$0.40  &91.95$\pm$0.39   &91.11$\pm$0.40   &89.72$\pm$0.39        &88.61$\pm$0.79    \\
                                                                                  
                                                            &                           & \cmark                                                                                   &\textbf{93.61$\pm$1.04}   &\textbf{92.78$\pm$1.04}   &\textbf{92.50$\pm$1.80}        &\textbf{91.67$\pm$2.96}  &\textbf{91.39$\pm$3.22}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &92.78$\pm$1.97  &88.61$\pm$1.42  &85.83$\pm$1.80   &79.72$\pm$2.83      &74.17$\pm$4.46                                   \\
                                                                                 &             & \cmark                                                     &\textbf{94.72$\pm$2.19}  &\textbf{92.22$\pm$3.75}   &\textbf{90.00$\pm$4.46}   &\textbf{86.11$\pm$4.10 }       &\textbf{79.17$\pm$4.91}                                                   \\ 
                                                    \bottomrule
\end{tabular}

\end{center}
\end{table}

==> tabs/appdix-tabs/handtype1.tex <==
%handwritten-type1
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type I).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.1}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.2}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.3}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.4}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}
\\ \midrule 
\multirow{17}{*} {\shortstack{\textbf{Hand-}\\\textbf{written}}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark          &97.18$\pm$1.92   &95.38$\pm$1.25   &93.34$\pm$1.31        &92.57$\pm$1.58       &91.28$\pm$1.31                          \\
                                                                                 &             & \cmark                                                                                                        &\textbf{98.46$\pm$1.26}  &\textbf{95.90$\pm$1.92}   &\textbf{93.85$\pm$1.88}   &\textbf{93.08$\pm$1.66}        &\textbf{92.31$\pm$0.63}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark          &88.46$\pm$1.66  &87.18$\pm$1.31   &86.92$\pm$1.09   &86.92$\pm$1.09        &86.92$\pm$1.09    \\
                                                                                  
                                                            &                           & \cmark                                                                                    &\textbf{90.77$\pm$3.33}  &\textbf{90.26$\pm$3.57}   &\textbf{89.75$\pm$3.85}   &\textbf{89.75$\pm$3.84}        &\textbf{89.75$\pm$3.84}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{3\}}}      & \xmark          &85.90$\pm$1.92   &85.13$\pm$1.81   &84.87$\pm$1.45        &84.62$\pm$1.66 &84.62$\pm$1.66                                 \\
                                                                                 &             & \cmark                                                                                                        &\textbf{88.97$\pm$2.54}  &\textbf{88.21$\pm$2.61}   &\textbf{87.69$\pm$2.74}   &\textbf{87.69$\pm$3.32}        &\textbf{87.44$\pm$3.10}                       \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark         &88.97$\pm$3.68   &83.08$\pm$3.50   &78.97$\pm$1.92        &77.69$\pm$2.74 &75.90$\pm$3.57                                 \\
                                                                                 &             & \cmark                                                     &\textbf{88.97$\pm$4.04}  &\textbf{83.59$\pm$2.97}   &\textbf{80.51$\pm$3.46}   &\textbf{77.18$\pm$4.28}        &\textbf{74.10$\pm$3.84}                       
                                                                                 \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 3\}}}      & \xmark          &91.54$\pm$1.09   &91.28$\pm$3.16   &88.97$\pm$5.41        &87.43$\pm$5.83 &85.64$\pm$6.42                                 \\
                                                                                 &             & \cmark                                                   &\textbf{93.59$\pm$2.38}  &\textbf{91.79$\pm$3.68}
                                        &\textbf{88.97$\pm$4.04}
                                     &\textbf{86.93$\pm$4.99}   &\textbf{85.39$\pm$4.91}                                                                          \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{2, 3\}}}      & \xmark          &63.59$\pm$8.00   &\textbf{59.74$\pm$7.00}   &\textbf{57.69$\pm$5.99}        &\textbf{56.67$\pm$5.94} &\textbf{55.90$\pm$5.49}                                 \\
                                                                                 &             & \cmark                                                              &\textbf{64.36$\pm$7.49}   &58.46$\pm$6.37   &56.67$\pm$6.10        &55.64$\pm$6.04 &54.87$\pm$6.29                                                                  \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2, 3\}}}      & \xmark          &54.87$\pm$10.68  &\textbf{37.95$\pm$6.92}   &\textbf{29.48$\pm$4.76}   &\textbf{24.36$\pm$4.04}        &\textbf{22.31$\pm$4.12}                                \\
                                                                                 &             & \cmark                                                     &\textbf{57.18$\pm$11.41}  &35.64$\pm$4.80   &26.67$\pm$2.54   &22.82$\pm$2.54        &20.77$\pm$1.09
                                                                                                              \\   \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tabs/appdix-tabs/handtype2.tex <==
%handwritten-type2
\begin{table}[ht]
\vskip 0.15in

\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type II).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.5}$\\ \end{tabular}}
\\ \midrule
\multirow{13}{*}  {\shortstack{\textbf{Hand-}\\\textbf{written}}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark          &98.42$\pm$0.51  &98.25$\pm$0.35   &97.92$\pm$0.12   &97.92$\pm$0.12        &97.58$\pm$0.12                                  \\
                                                                                 &             & \cmark                &\textbf{99.50$\pm$0.41}   &\textbf{99.50$\pm$0.41}   &\textbf{99.50$\pm$0.41}        &\textbf{99.50$\pm$0.41}  &\textbf{99.50$\pm$0.41}                                      \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark          &98.17$\pm$1.03  &97.75$\pm$0.54   &97.33$\pm$0.47   &97.00$\pm$0.41        &96.92$\pm$0.42    \\
                                                                                  
                                                            &                           & \cmark                                                                                  &\textbf{98.83$\pm$0.24}   &\textbf{98.50$\pm$0.41}   &\textbf{98.67$\pm$0.47}        &\textbf{98.67$\pm$0.47}  &\textbf{98.67$\pm$0.47}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &97.67$\pm$0.47  &97.25$\pm$0.54  &96.58$\pm$0.51  &95.92$\pm$0.59   &95.67$\pm$0.94                                         \\
                                                                                 &             & \cmark                                             &\textbf{99.00$\pm$0.00}  &\textbf{98.83$\pm$0.24}   &\textbf{98.83$\pm$0.24}   &\textbf{98.83$\pm$0.24}       &\textbf{98.83$\pm$0.24}                                                                                                      \\ 
  \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 3\}}}      & \xmark          &98.08$\pm$0.12   &97.00$\pm$1.22   &96.33$\pm$1.55        &95.33$\pm$1.55       &95.08$\pm$1.59                           \\
                                                                                 &             & \cmark                                                     &\textbf{99.50$\pm$0.00}  &\textbf{99.17$\pm$0.47}   &\textbf{98.00$\pm$0.41}   &\textbf{97.67$\pm$0.24}        &\textbf{95.78$\pm$1.04}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2, 3\}}}       & \xmark         &98.17$\pm$0.24  &96.83$\pm$0.47   &95.67$\pm$0.85   &94.75$\pm$0.94        &94.17$\pm$0.85    \\
                                                                                  
                                                            &                           & \cmark                                                                                    &\textbf{99.00$\pm$0.00}  &\textbf{98.67$\pm$0.47}   &\textbf{97.67$\pm$0.62}   &\textbf{97.33$\pm$1.03}        &\textbf{97.33$\pm$1.03}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2, 3\}}}      & \xmark          &96.50$\pm$1.08   &93.58$\pm$1.74   &90.67$\pm$3.09        &88.75$\pm$3.54 &87.58$\pm$3.36                                 \\
                                                                                 &             & \cmark                                                     &\textbf{98.50$\pm$0.71}  &\textbf{97.17$\pm$1.18}   &\textbf{95.50$\pm$1.22}   &\textbf{93.67$\pm$0.85}        &\textbf{92.50$\pm$0.82}                                                                                        \\   
  
                             \bottomrule
\end{tabular}

\end{center}
\end{table}


==> tabs/appdix-tabs/tuandtype1.tex <==
%TUANDROMD
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type I).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.1}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.2}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.3}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.4}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}
\\ \midrule 
\multirow{7}{*} {\shortstack{\textbf{TUAND-}\\\textbf{ROMD}}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark          &84.77$\pm$0.55                                                    &80.47$\pm$0.99  &76.53$\pm$1.11   &72.65$\pm$0.76   &70.17$\pm$0.66                                          \\
                                                                                 &             & \cmark               &\textbf{86.50$\pm$0.59}               &\textbf{82.46$\pm$0.77}   &\textbf{78.30$\pm$1.18}   &\textbf{74.92$\pm$1.39}        &\textbf{72.45$\pm$1.33}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark                                                              &86.56$\pm$0.27  &85.71$\pm$0.48   &84.14$\pm$0.58   &82.35$\pm$0.86        &80.85$\pm$1.05    \\
                                                                                  
                                                            &                           & \cmark                                                                                   &\textbf{88.87$\pm$0.22}               &\textbf{88.74$\pm$0.28}   &\textbf{88.58$\pm$0.63}   &\textbf{88.15$\pm$0.65}        &\textbf{87.93$\pm$0.67}                                          \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &84.88$\pm$1.19                                                    &80.72$\pm$1.02  &76.60$\pm$0.75  &73.15$\pm$1.10  &70.35$\pm$1.25                                            \\
                                                                                 &             & \cmark                                                    &\textbf{87.41$\pm$3.40}                                                    &\textbf{82.78$\pm$1.14}  &\textbf{79.28$\pm$1.00}   &\textbf{76.30$\pm$1.11}   &\textbf{73.82$\pm$1.35}                                                                                                             \\ 
                                                    \bottomrule
\end{tabular}

\end{center}
\end{table}


==> tabs/appdix-tabs/tuandtype2.tex <==
%TUANDROMD
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type II).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.5}$\\ \end{tabular}}
\\ \midrule
\multirow{7}{*} {\shortstack{\textbf{TUAND-}\\\textbf{ROMD}}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark          &81.14$\pm$0.70                                                    &78.21$\pm$0.92  &75.39$\pm$1.09   &73.21$\pm$1.46   &71.71$\pm$1.26                                          \\
                                                                                 &             & \cmark                            &\textbf{81.99$\pm$1.99}   &\textbf{78.79$\pm$2.42}   &\textbf{76.37$\pm$2.57}        &\textbf{74.36$\pm$2.63}      &\textbf{73.19$\pm$2.60}
                                                                                 \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark                                                              &84.19$\pm$0.82  &84.43$\pm$0.48  &84.46$\pm$0.35 &84.32$\pm$0.45   &84.21$\pm$0.44            \\
                                                                                  
                                                            &                           & \cmark                                                                                   &\textbf{84.88$\pm$1.62}               &\textbf{84.73$\pm$1.89}   &\textbf{84.84$\pm$1.76}   &\textbf{84.39$\pm$0.89}        &\textbf{84.97$\pm$1.52}                                          \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &83.56$\pm$1.23                                                    &80.85$\pm$1.30  &77.85$\pm$1.53  &75.90$\pm$2.07  &74.08$\pm$2.22                                            \\
                                                                                 &             & \cmark                                                    &\textbf{83.99$\pm$1.87}                 &\textbf{81.48$\pm$2.30}  &\textbf{78.50$\pm$2.30}   &\textbf{76.73$\pm$2.19}   &\textbf{75.23$\pm$2.20}                                                                                                             \\ 
                                                    \bottomrule
\end{tabular}

\end{center}
\end{table}


==> tabs/appdix-tabs/yalebtype1.tex <==
%yaleB-type1
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type I).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.1}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.2}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.3}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.4}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}
\\ \midrule 
\multirow{17}{*} {\textbf{YaleB}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark                                                                 &97.43$\pm$1.58   &96.92$\pm$1.88   &96.41$\pm$2.20        &94.10$\pm$1.31       &92.82$\pm$1.31                          \\
                                                                                 &             & \cmark                                                                    &\textbf{98.46$\pm$1.09}  &\textbf{98.20$\pm$1.31}   &\textbf{96.15$\pm$1.88}   &\textbf{94.62$\pm$1.88}        &\textbf{93.59$\pm$1.30}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark                                                              &95.13$\pm$0.72  &94.10$\pm$1.31   &92.57$\pm$0.73   &92.05$\pm$1.45        &91.54$\pm$1.66    \\
                                                                                  
                                                            &                           & \cmark                                                                                                   &\textbf{96.92$\pm$1.26}  &\textbf{95.90$\pm$2.02}
                                       &\textbf{94.61$\pm$2.88} &\textbf{93.33$\pm$2.54}   &\textbf{93.08$\pm$3.14}                \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{3\}}}      & \xmark                                                                &94.87$\pm$0.96   &94.87$\pm$0.96   &94.10$\pm$0.96        &92.82$\pm$1.81 &92.05$\pm$1.31                                 \\
                                                                                 &             & \cmark                                                                                                      &\textbf{96.92$\pm$1.88}  &\textbf{97.18$\pm$1.92}   &\textbf{96.15$\pm$1.88}   &\textbf{94.87$\pm$2.54}        &\textbf{94.36$\pm$2.02}                       \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark             &96.67$\pm$2.61   &95.13$\pm$3.46   &91.28$\pm$2.83        &88.72$\pm$3.10 &86.41$\pm$3.10                                 \\
                                                                                 &             & \cmark                                                                &\textbf{97.69$\pm$0.63}  &\textbf{95.39$\pm$2.26}   &\textbf{92.56$\pm$2.02}   &\textbf{89.72$\pm$2.21}        &\textbf{86.66$\pm$1.81}                       
                                                                                 \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 3\}}}      & \xmark          &97.43$\pm$0.96   &97.69$\pm$1.66   &97.43$\pm$1.81        &97.18$\pm$2.20 &96.15$\pm$2.26                                 \\
                                                                                 &             & \cmark                                                    &\textbf{98.46$\pm$1.09}  &\textbf{98.46$\pm$1.26}
                                       &\textbf{98.46$\pm$1.66}
                                       &\textbf{96.92$\pm$1.88}    &\textbf{96.67$\pm$2.20}                                                                          \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{2, 3\}}}      & \xmark      &94.62$\pm$1.08   &93.85$\pm$1.25   &90.26$\pm$2.54        &87.95$\pm$2.83 &86.67$\pm$2.38                                 \\
                                                                                 &             & \cmark                       &\textbf{96.41$\pm$1.81}   
                                       &\textbf{95.64$\pm$1.92}   
                                       &\textbf{93.84$\pm$3.32}    
                                       &\textbf{91.28$\pm$3.10} 
                                       &\textbf{89.49$\pm$3.16}                         \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2, 3\}}}      & \xmark          &96.15$\pm$1.88  &96.41$\pm$3.16   &93.85$\pm$4.40   &87.69$\pm$8.21        &84.10$\pm$10.32                                \\
                                                                                 &             & \cmark     &\textbf{97.43$\pm$1.81}  &\textbf{97.43$\pm$1.92}   &\textbf{93.85$\pm$4.40}   &\textbf{87.69$\pm$7.61}        &\textbf{82.56$\pm$9.26}
                                                                                                              \\   \bottomrule
\end{tabular}
\end{center}
\end{table}

==> tabs/appdix-tabs/yalebtype2.tex <==
%yaleB-type2
\begin{table}[ht]
\vskip 0.15in
\begin{center}
\footnotesize
\caption{Accuracy performance comparison when some of the modalities is blurred (Type II).}
\center
\setlength{\tabcolsep}{ 1.11mm}\begin{tabular}{c|cc|ccccc}
\toprule
\textbf{Dataset}  & \textbf{Noise on}  & \textbf{MCCA}  &
\textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=0.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=1.5}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.0}$\\ \end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}$\mathbf{\epsilon=2.5}$\\ \end{tabular}}
\\ \midrule
\multirow{17}{*} {\textbf{YaleB}}  
     &  \multirow{2}{*}{\text{\{1\}}}      & \xmark   &95.90$\pm$2.54   &94.87$\pm$3.22        &93.85$\pm$2.88       &93.59$\pm$3.16       &93.59$\pm$3.16                   \\
                                                                                 &             & \cmark                                                     &\textbf{97.43$\pm$1.31}  &\textbf{96.15$\pm$2.51}   &\textbf{95.13$\pm$2.97}   &\textbf{94.36$\pm$2.97}        &\textbf{93.85$\pm$3.46}                                        \\ \cmidrule{2-8}
      &  \multirow{2}{*}{\text{\{2\}}}       & \xmark          &96.15$\pm$2.26  &93.33$\pm$3.22   &91.03$\pm$2.62   &90.26$\pm$2.02        &89.23$\pm$2.18    \\
                                                                                  
                                                            &                           & \cmark                                                                                    &\textbf{97.69$\pm$1.26}  &\textbf{96.67$\pm$1.58}   &\textbf{94.10$\pm$2.20}   &\textbf{92.82$\pm$2.83}        &\textbf{92.05$\pm$2.02}                                        \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{3\}}}      & \xmark &98.72$\pm$0.36   &96.92$\pm$1.26   &96.15$\pm$0.63        &96.15$\pm$0.63 &95.90$\pm$0.96                                 \\
                                                                                 &             & \cmark                                                    &\textbf{98.72$\pm$0.73}  &\textbf{97.69$\pm$1.09}   &\textbf{97.43$\pm$0.96}   &\textbf{97.18$\pm$1.31}        &\textbf{96.67$\pm$1.58}                       \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2\}}}      & \xmark          &95.64$\pm$2.83   &91.02$\pm$3.46        &88.46$\pm$4.53 &87.18$\pm$3.46      &85.90$\pm$4.09                           \\
                                                                                 &             & \cmark                                                     &\textbf{96.66$\pm$1.31}   &\textbf{93.59$\pm$2.38}        &\textbf{90.51$\pm$2.97} &\textbf{86.67$\pm$3.46}      &\textbf{84.62$\pm$3.26}                       
                                                                                 \\ \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 3\}}}      & \xmark          &98.46$\pm$0.63   &98.46$\pm$1.66   &97.69$\pm$1.66        &97.43$\pm$1.45 &97.18$\pm$1.31                                 \\
                                                                                 &             & \cmark                                                     &\textbf{98.20$\pm$0.73}  &\textbf{97.95$\pm$1.92}
                                        &\textbf{97.69$\pm$1.66}
                                     &\textbf{98.20$\pm$1.58}   &\textbf{97.69$\pm$1.66}                                                                          \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{2, 3\}}}      & \xmark          &97.43$\pm$0.36   &95.89$\pm$0.36   &95.38$\pm$0.62        &94.62$\pm$0.62 &92.82$\pm$0.73                                 \\
                                                                                 &             & \cmark                                                    &\textbf{98.72$\pm$0.36}   &\textbf{97.69$\pm$1.09}   &\textbf{96.66$\pm$0.73}        &\textbf{95.38$\pm$0.62} &\textbf{94.61$\pm$1.66}                                                                  \\
                                                                                 \cmidrule{2-8}
     &  \multirow{2}{*}{\text{\{1, 2, 3\}}}      & \xmark          &97.69$\pm$0.63  &95.64$\pm$0.36   &93.08$\pm$1.09   &89.23$\pm$1.66        &82.31$\pm$1.26                                \\
                                                                                 &             & \cmark                              &\textbf{98.46$\pm$0.63}  &\textbf{97.18$\pm$1.31}   &\textbf{95.64$\pm$0.96}   &\textbf{92.56$\pm$2.54}        &\textbf{88.46$\pm$2.27}
                                                                                                              \\   \bottomrule
\end{tabular}
\end{center}
\end{table}
